DeBaCl: A Python Package for Interactive DEnsity-BAsed CLustering

The level set tree approach of Hartigan (1975) provides a probabilistically based and highly interpretable encoding of the clustering behavior of a dataset. By representing the hierarchy of data modes as a dendrogram of the level sets of a density estimator, this approach offers many advantages for exploratory analysis and clustering, especially for complex and high-dimensional data. Several R packages exist for level set tree estimation, but their practical usefulness is limited by computational inefficiency, absence of interactive graphical capabilities and, from a theoretical perspective, reliance on asymptotic approximations. To make it easier for practitioners to capture the advantages of level set trees, we have written the Python package DeBaCl for DEnsity-BAsed CLustering. In this article we illustrate how DeBaCl's level set tree estimates can be used for difficult clustering tasks and interactive graphical data analysis. The package is intended to promote the practical use of level set trees through improvements in computational efficiency and a high degree of user customization. In addition, the flexible algorithms implemented in DeBaCl enjoy finite sample accuracy, as demonstrated in recent literature on density clustering. Finally, we show the level set tree framework can be easily extended to deal with functional data.

==> tex_source/extensions.tex <==


%% This file was auto-generated by IPython.
%% Conversion from the original notebook file:
%%
%\documentclass[11pt,english]{article}

%% This is the automatic preamble used by IPython.  Note that it does *not*
%% include a documentclass declaration, that is added at runtime to the overall
%% document.

%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{graphicx}
%\usepackage{ucs}
%\usepackage[utf8x]{inputenc}
%\usepackage{caption}
%\usepackage{subcaption}

% needed for markdown enumerations to work
%\usepackage{enumerate}

% Slightly bigger margins than the latex defaults
%\usepackage{geometry}
%\geometry{verbose,tmargin=3cm,bmargin=3cm,lmargin=2.5cm,rmargin=2.5cm}

% Define a few colors for use in code, links and cell shading
%\usepackage{color}
%\definecolor{orange}{cmyk}{0,0.4,0.8,0.2}
%\definecolor{darkorange}{rgb}{.71,0.21,0.01}
%\definecolor{darkgreen}{rgb}{.12,.54,.11}
%\definecolor{myteal}{rgb}{.26, .44, .56}
%\definecolor{gray}{gray}{0.45}
%\definecolor{lightgray}{gray}{.95}
%\definecolor{mediumgray}{gray}{.8}
%\definecolor{inputbackground}{rgb}{.95, .95, .85}
%\definecolor{outputbackground}{rgb}{.95, .95, .95}
%\definecolor{traceback}{rgb}{1, .95, .95}

% Framed environments for code cells (inputs, outputs, errors, ...).  The
% various uses of \unskip (or not) at the end were fine-tuned by hand, so don't
% randomly change them unless you're sure of the effect it will have.
%\usepackage{framed}

% remove extraneous vertical space in boxes
%\setlength\fboxsep{0pt}

% codecell is the whole input+output set of blocks that a Code cell can
% generate.

% TODO: unfortunately, it seems that using a framed codecell environment breaks
% the ability of the frames inside of it to be broken across pages.  This
% causes at least the problem of having lots of empty space at the bottom of
% pages as new frames are moved to the next page, and if a single frame is too
% long to fit on a page, will completely stop latex from compiling the
% document.  So unless we figure out a solution to this, we'll have to instead
% leave the codecell env. as empty.  I'm keeping the original codecell
% definition here (a thin vertical bar) for reference, in case we find a
% solution to the page break issue.

%% \newenvironment{codecell}{%
%%     \def\FrameCommand{\color{mediumgray} \vrule width 1pt \hspace{5pt}}%
%%    \MakeFramed{\vspace{-0.5em}}}
%%  {\unskip\endMakeFramed}

% For now, make this a no-op...
%\newenvironment{codecell}{}

% \newenvironment{codeinput}{%
%   \def\FrameCommand{\colorbox{inputbackground}}%
%   \MakeFramed{\advance\hsize-\width \FrameRestore}}
% {\unskip\endMakeFramed}

%\newenvironment{codeoutput}{%
%   \def\FrameCommand{\colorbox{outputbackground}}%
%   \vspace{-1.4em}
%   \MakeFramed{\advance\hsize-\width \FrameRestore}}
% {\unskip\medskip\endMakeFramed}

%\newenvironment{traceback}{%
%   \def\FrameCommand{\colorbox{traceback}}%
%   \MakeFramed{\advance\hsize-\width \FrameRestore}}
% {\endMakeFramed}

% Use and configure listings package for nicely formatted code
%\usepackage{listingsutf8}
%\lstset{
%  language=python,
%  inputencoding=utf8x,
%  extendedchars=\true,
%  aboveskip=\smallskipamount,
%  belowskip=\smallskipamount,
%  xleftmargin=2mm,
%  breaklines=true,
%  basicstyle=\small \ttfamily,
%  showstringspaces=false,
%  keywordstyle=\color{blue}\bfseries,
%  commentstyle=\color{myteal},
%  stringstyle=\color{darkgreen},
%  identifierstyle=\color{darkorange},
%  columns=fullflexible,  % tighter character kerning, like verb
%}

% The hyperref package gives us a pdf with properly built
% internal navigation ('pdf bookmarks' for the table of contents,
% internal cross-reference links, web links for URLs, etc.)
%\usepackage{hyperref}
%\hypersetup{
%  breaklinks=true,  % so long urls are correctly broken across lines
%  colorlinks=true,
%  urlcolor=blue,
%  linkcolor=darkorange,
%  citecolor=darkgreen,
%  }

% hardcode size of all verbatim environments to be a bit smaller
%\makeatletter 
%\g@addto@macro\@verbatim\small\topsep=0.5em\partopsep=0pt
%\makeatother 

% Prevent overflowing lines due to urls and other hard-to-break entities.
%\sloppy




%\begin{document}


\begin{codecell}
\begin{codeinput}
\begin{lstlisting}
## Import DeBaCl package
import debacl as dcl
import gen_utils as utl
import plot_utils as plutl
import cd_tree as cdt

## Other python libraries
import numpy as np

## Load the data
X = np.loadtxt('0187_endpoints.csv', delimiter=',')
n, p = X.shape

## Downsample because exact Chaudhuri-Dasgupta is super slow
ix_keep = np.random.choice(range(n), size=200, replace=False)
X = X[ix_keep, :]
n, p = X.shape
\end{lstlisting}
\end{codeinput}

\end{codecell}
\begin{codecell}
\begin{codeinput}
\begin{lstlisting}
p_k = 0.01
k = int(p_k * n)
p_gamma = 0.05

tree = cdt.makeCDTree(X, k, start='max-radius', verbose=True) 
\end{lstlisting}
\end{codeinput}
\begin{codeoutput}

\begin{verbatim}
iteration: 0 / 4318
iteration: 1000 / 4318
iteration: 2000 / 4318
iteration: 3000 / 4318
iteration: 4000 / 4318

\end{verbatim}

\end{codeoutput}
\end{codecell}
\begin{codecell}
\begin{codeinput}
\begin{lstlisting}
speech = np.loadtxt('smooth_phoneme.csv', delimiter=',')
phoneme = speech[:, -1].astype(np.int)
speech = speech[:, :-1]

n, p = speech.shape
print "n:", n, "\np:", p
print "Phoneme counts:", np.bincount(phoneme)
\end{lstlisting}
\end{codeinput}
\begin{codeoutput}

\begin{verbatim}
n: 2000 
p: 150
Phoneme counts: [400 400 400 400 400]

\end{verbatim}

\end{codeoutput}
\end{codecell}
\begin{codecell}
\begin{codeinput}
\begin{lstlisting}
## Output libraries and formatting
import matplotlib.pyplot as plt
from mpl_toolkits.mplot3d import Axes3D
import matplotlib as mpl
from matplotlib import ticker

mpl.rc('axes', labelsize=16)
mpl.rc('xtick', labelsize=11)
mpl.rc('ytick', labelsize=11)
#mpl.rc('savefig', dpi=200)

def autoloc(self):
	ticker.MaxNLocator.__init__(self, nbins=4)
ticker.AutoLocator.__init__ = autoloc
\end{lstlisting}
\end{codeinput}

\end{codecell}
\begin{codecell}
\begin{codeinput}
\begin{lstlisting}
fig, ax = plt.subplots(3, 2, sharex=True, sharey=True)
ax = ax.flatten()
ax[-2].set_xlabel('frequencies')
ax[-1].set_xlabel('frequencies')

for g in np.unique(phoneme):
	ix = np.where(phoneme == g)[0]
	for j in ix:
		ax[g].plot(speech[j, :], c='black', alpha=0.15)
        
fig.savefig('../figures/phoneme_data.png')
\end{lstlisting}
\end{codeinput}

\end{codecell}
\begin{figure}
    \centering
    \includegraphics[width=0.65\textwidth]{figures/phoneme_data.png}
    \caption{Smoothed waveforms for spoken phonemes, separated by true phoneme.}
    \label{fig:phoneme_data}
\end{figure}




%\end{document}


